Complete Heyting Algebra Semantics for an Intuitionistic Version of Matching Logic (Extended Abstract)

We present work in progress towards an intuitionistic version of Applicative Matching Logic. We introduce a semantics based on complete Heyting algebras, and propose a proof system which we prove to be sound relative to this semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{217}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.14}{10.4204/EPTCS.452.14}}

